Space-Efficient Gradual Typing in Coercion-Passing Style

Herman et al. pointed out that the insertion of run-time checks into a gradually typed program could hamper tail-call optimization and, as a result, worsen the space complexity of the program. To address the problem, they proposed a space-efficient coercion calculus, which was subsequently improved by Siek et al. The semantics of these calculi involves eager composition of run-time checks expressed by coercions to prevent the size of a term from growing. However, it relies also on a nonstandard reduction rule, which does not seem easy to implement. In fact, no compiler implementation of gradually typed languages fully supports the space-efficient semantics faithfully. In this paper, we study coercion-passing style, which Herman et al. have already mentioned, as a technique for straightforward space-efficient implementation of gradually typed languages. A program in coercion-passing style passes "the rest of the run-time checks" around---just like continuation-passing style (CPS), in which "the rest of the computation" is passed around---and (unlike CPS) composes coercions eagerly. We give a formal coercion-passing translation from $\lambda$S by Siek et al. to $\lambda$S$_1$, which is a new calculus of first-class coercions tailored for coercion-passing style, and prove correctness of the translation. We also implement our coercion-passing style transformation for the Grift compiler developed by Kuhlenschmidt et al. An experimental result shows stack overflow can be prevented properly at the cost of up to 3 times slower execution for most partially typed practical programs.

==> figure/semS.tex <==
\begin{figure}[tb]
  \begin{align*}
    \text{Evaluation contexts}&&
    \mathcal{E} &\grmeq
    \mathcal{F} \grmor
    \mathcal{F}  [  \square \, \langle  \ottnt{s}  \rangle  ]
    \\
    &&
    \mathcal{F} &\grmeq
    \graytext{
       \square  \grmor
      \mathcal{E}  [  \ottnt{op}  \ottsym{(}  \square  \ottsym{,}  \ottnt{M}  \ottsym{)}  ] \grmor
      \mathcal{E}  [  \ottnt{op}  \ottsym{(}  \ottnt{V}  \ottsym{,} \, \square \, \ottsym{)}  ] \grmor
      \mathcal{E}  [  \square \, \ottnt{M}  ] \grmor
      \mathcal{E}  [  \ottnt{V} \, \square  ]
    }
  \end{align*}
  Coercion composition \hfill\fbox{$\ottnt{s}  \fatsemi  \ottnt{t}  \ottsym{=}  \ottnt{s'}$}
  \begin{align*}
     \ottkw{id} _{ \mathord{\star} }   \fatsemi  \ottnt{t} &= \ottnt{t} &\rn{CC-IdDynL}\\
    \ottsym{(}   \ottnt{G} \texttt{?}^{ \ottnt{p} }   \ottsym{;}  \ottnt{i}  \ottsym{)}  \fatsemi  \ottnt{t} &=  \ottnt{G} \texttt{?}^{ \ottnt{p} }   \ottsym{;}  \ottsym{(}  \ottnt{i}  \fatsemi  \ottnt{t}  \ottsym{)} &\rn{CC-ProjL}\\[0.5em]
    \ottsym{(}  \ottnt{g}  \ottsym{;}   \ottnt{G} \texttt{!}   \ottsym{)}  \fatsemi   \ottkw{id} _{ \mathord{\star} }  &= \ottnt{g}  \ottsym{;}   \ottnt{G} \texttt{!}  &\rn{CC-InjId}\\
    \ottsym{(}  \ottnt{g}  \ottsym{;}   \ottnt{G} \texttt{!}   \ottsym{)}  \fatsemi  \ottsym{(}   \ottnt{G} \texttt{?}^{ \ottnt{p} }   \ottsym{;}  \ottnt{i}  \ottsym{)} &= \ottnt{g}  \fatsemi  \ottnt{i} &\rn{CC-Collapse}\\
    \ottsym{(}  \ottnt{g}  \ottsym{;}   \ottnt{G} \texttt{!}   \ottsym{)}  \fatsemi  \ottsym{(}   \ottnt{H} \texttt{?}^{ \ottnt{p} }   \ottsym{;}  \ottnt{i}  \ottsym{)} &=  \bot^{ \ottnt{G}   \ottnt{p}   \ottnt{H} } 
    \text{\hspace{5.7em} if $\ottnt{G}  \ne  \ottnt{H}$} &\rn{CC-Conflict}\\
     \bot^{ \ottnt{G}   \ottnt{p}   \ottnt{H} }   \fatsemi  \ottnt{s} &=  \bot^{ \ottnt{G}   \ottnt{p}   \ottnt{H} }  &\rn{CC-FailL}\\[0.5em]
    \ottnt{g}  \fatsemi   \bot^{ \ottnt{G}   \ottnt{p}   \ottnt{H} }  &=  \bot^{ \ottnt{G}   \ottnt{p}   \ottnt{H} }  &\rn{CC-FailR}\\
    \ottnt{g}  \fatsemi  \ottsym{(}  \ottnt{h}  \ottsym{;}   \ottnt{H} \texttt{!}   \ottsym{)} &= \ottsym{(}  \ottnt{g}  \fatsemi  \ottnt{h}  \ottsym{)}  \ottsym{;}   \ottnt{H} \texttt{!}  &\rn{CC-InjR}\\[0.5em]
     \ottkw{id} _{ \ottnt{A} }   \fatsemi  \ottnt{g} &= \ottnt{g} \text{\hspace{7.4em} if $\ottnt{A}  \ne  \mathord{\star}$} &\rn{CC-IdL}\\
    \ottnt{g}  \fatsemi   \ottkw{id} _{ \ottnt{A} }  &= \ottnt{g} \text{\hspace{7.4em} if $\ottnt{A}  \ne  \mathord{\star}$ and $\ottnt{g}  \ne   \ottkw{id} _{ \ottnt{A} } $} &\rn{CC-IdR}\\
    \ottsym{(}  \ottnt{s}  \rightarrow  \ottnt{t}  \ottsym{)}  \fatsemi  \ottsym{(}  \ottnt{s'}  \rightarrow  \ottnt{t'}  \ottsym{)} &= \begin{cases}
       \ottkw{id} _{ \ottnt{A}  \rightarrow  \ottnt{B} }  &\text{if $\ottnt{s'}  \fatsemi  \ottnt{s}  \ottsym{=}   \ottkw{id} _{ \ottnt{A} } $ and $\ottnt{t}  \fatsemi  \ottnt{t'}  \ottsym{=}   \ottkw{id} _{ \ottnt{B} } $} \\
      \ottsym{(}  \ottnt{s'}  \fatsemi  \ottnt{s}  \ottsym{)}  \rightarrow  \ottsym{(}  \ottnt{t}  \fatsemi  \ottnt{t'}  \ottsym{)} &\text{otherwise}
    \end{cases} &\rn{CC-Fun}
  \end{align*}
  Reduction \hfill\fbox{$ \ottnt{M}    \mathbin{\accentset{\mathsf{e} }{\reduces}_{\mathsf{S} } }    \ottnt{N} $}\quad\fbox{$ \ottnt{M}    \mathbin{\accentset{\mathsf{c} }{\reduces}_{\mathsf{S} } }    \ottnt{N} $}
  \begin{align*}
    \ottnt{op}  \ottsym{(}  \ottnt{a}  \ottsym{,}  \ottnt{b}  \ottsym{)} & \mathbin{\accentset{\mathsf{e} }{\reduces} }  \delta \, \ottsym{(}  \ottnt{op}  \ottsym{,}  \ottnt{a}  \ottsym{,}  \ottnt{b}  \ottsym{)} &\rn{R-Op} \\
    \ottsym{(}   \lambda   \ottmv{x} .\,  \ottnt{M}   \ottsym{)} \, \ottnt{V} & \mathbin{\accentset{\mathsf{e} }{\reduces} }  \ottnt{M}  [  \ottmv{x}  \ottsym{:=}  \ottnt{V}  ] &\rn{R-Beta}\\
    \ottsym{(}  \ottnt{U}  \langle\!\langle  \ottnt{s}  \rightarrow  \ottnt{t}  \rangle\!\rangle  \ottsym{)} \, \ottnt{V} & \mathbin{\accentset{\mathsf{e} }{\reduces} }  \ottsym{(}  \ottnt{U} \, \ottsym{(}  \ottnt{V}  \langle  \ottnt{s}  \rangle  \ottsym{)}  \ottsym{)}  \langle  \ottnt{t}  \rangle &\rn{R-Wrap} \\
    \ottnt{U}  \langle   \ottkw{id} _{ \ottnt{A} }   \rangle & \mathbin{\accentset{\mathsf{c} }{\reduces} }  \ottnt{U} &\rn{R-Id} \\
    \ottnt{U}  \langle   \bot^{ \ottnt{G}   \ottnt{p}   \ottnt{H} }   \rangle & \mathbin{\accentset{\mathsf{c} }{\reduces} }  \ottkw{blame} \, \ottnt{p} &\rn{R-Fail}\\
    \ottnt{U}  \langle  \ottnt{d}  \rangle & \mathbin{\accentset{\mathsf{c} }{\reduces} }  \ottnt{U}  \langle\!\langle  \ottnt{d}  \rangle\!\rangle &\rn{R-Crc} \\
    \ottnt{M}  \langle  \ottnt{s}  \rangle  \langle  \ottnt{t}  \rangle & \mathbin{\accentset{\mathsf{c} }{\reduces} }  \ottnt{M}  \langle  \ottnt{s}  \fatsemi  \ottnt{t}  \rangle &\rn{R-MergeC}\\
    \ottnt{U}  \langle\!\langle  \ottnt{d}  \rangle\!\rangle  \langle  \ottnt{t}  \rangle & \mathbin{\accentset{\mathsf{c} }{\reduces} }  \ottnt{U}  \langle  \ottnt{d}  \fatsemi  \ottnt{t}  \rangle &\rn{R-MergeV}
  \end{align*}
  Evaluation \hfill\fbox{$ \ottnt{M}    \mathbin{  \accentset{\mathsf{e} }{\evalto}_{\mathsf{S_1} }  }    \ottnt{N} $}\quad\fbox{$ \ottnt{M}    \mathbin{  \accentset{\mathsf{c} }{\evalto}_{\mathsf{S_1} }  }    \ottnt{N} $}
  \begin{center}
    \infrule[E-CtxE]{
       \ottnt{M}    \mathbin{\accentset{\mathsf{e} }{\reduces} }    \ottnt{N} 
    }{
       \mathcal{E}  [  \ottnt{M}  ]    \mathbin{  \accentset{\mathsf{e} }{\evalto}  }    \mathcal{E}  [  \ottnt{N}  ] 
    } \hgap
    \infrule[E-CtxC]{
       \ottnt{M}    \mathbin{\accentset{\mathsf{c} }{\reduces} }    \ottnt{N} 
    }{
       \mathcal{F}  [  \ottnt{M}  ]    \mathbin{  \accentset{\mathsf{c} }{\evalto}  }    \mathcal{F}  [  \ottnt{N}  ] 
    } \hgap
    \infrule[E-Abort]{
      \mathcal{E}  \ne  \square
    }{
       \mathcal{E}  [  \ottkw{blame} \, \ottnt{p}  ]    \mathbin{  \accentset{\mathsf{e} }{\evalto}  }    \ottkw{blame} \, \ottnt{p} 
    }
  \end{center}
  \caption{Reduction/evaluation rules of \lamS.}
  \label{fig:semS}
\end{figure}

